Deep metric learning improves lab of origin prediction of genetically engineered plasmids

Genome engineering is undergoing unprecedented development and is now becoming widely available. To ensure responsible biotechnology innovation and to reduce misuse of engineered DNA sequences, it is vital to develop tools to identify the lab-of-origin of engineered plasmids. Genetic engineering attribution (GEA), the ability to make sequence-lab associations, would support forensic experts in this process. Here, we propose a method, based on metric learning, that ranks the most likely labs-of-origin whilst simultaneously generating embeddings for plasmid sequences and labs. These embeddings can be used to perform various downstream tasks, such as clustering DNA sequences and labs, as well as using them as features in machine learning models. Our approach employs a circular shift augmentation approach and is able to correctly rank the lab-of-origin $90\%$ of the time within its top 10 predictions - outperforming all current state-of-the-art approaches. We also demonstrate that we can perform few-shot-learning and obtain $76\%$ top-10 accuracy using only $10\%$ of the sequences. This means, we outperform the previous CNN approach using only one-tenth of the data. We also demonstrate that we are able to extract key signatures in plasmid sequences for particular labs, allowing for an interpretable examination of the model's outputs.

==> tex/related_work.tex <==
\section{Related Work}

\subsection{Genetic Engineering Attribution}
Detecting genetic modifications and attributing them to a specific origin is a recent and open problem. Tools have been developed for detecting genetic engineering through genetic analysis of the organism genome. This is the case of FELIX (Finding Engineering-Linked Indicators) \cite{felix}, a program developed by IARPA that can rapidly detect indicators of genome engineering and has recently demonstrated its power by demystifying the rumors that the COVID-19 virus was created in a laboratory. However, assigning the origin of a specific engineered DNA to a lab is a more complex challenge.

For this task, machine learning has been used based on its capacity of recognizing patterns, an essential characteristic for detecting signatures inside a genome. The first attempt was made by \citeauthor{Nielsen2018} in 2018 when they used deep learning by applying convolutional neural networks. This network was trained on the Addgene plasmid dataset, presented in this work as well, where the authors collected several sequences of engineered DNA  in large public and private repositories. They treated the DNA sequence as a one-hot encoded vector, using it as input to the network composed of one convolutional layer of 128 filters, max-pooling operation, and two dense layers. Despite they show it's possible to use machine learning for this task, this first work got a low accuracy of 48\% correctly predicting the lab-of-origin. 

Later, in 2020, \citeauthor{Alley2020} demonstrated a recurrent network, which they called deteRNNt, capable of correctly assigning specific engineering DNA to more than 1,300 laboratories 70\% of the time. This represented a great improvement in the performance of a machine learning model applied to this task, surpassing by more than 20\% the previous work and with far more laboratory options to be distinguished.  The main difference of this work was to treat the DNA sequence as a text problem, using techniques from the natural language processing field to extract features from the sequence. They tokenized the sequence using Byte Pair Encoding \cite{gage1994}, generating larger tokens and decreasing the size of the sequence. These tokens then served as input to a word embedding layer \cite{wordembedding} followed by recurrent neural networks \cite{rnn1} \cite{rnn2}. 



\subsection{Metric Learning}


Metric Learning aims to automate learning task-specific distance functions in a (weakly) supervised manner \cite{kulis2013}. The goal is to learn a distance metric to compare two data points for how similar or distant they are. We can use these learned distance functions to perform various tasks, including clustering, information retrieval, identification, etc. One of the most well-known applications is Face Recognition \cite{liu2017} \cite{deng2018} \cite{wang2017} \cite{wang2018} \cite{wang2018_2}, in which we can compare a face with a reference picture and match them if they are similar enough.

The most common output when training a model for Metric Learning is what we call an embedding. Embedding is a vectorial representation of some entity composed of latent features. We can then apply well-known distance/similarity functions like euclidean distance to compare a pair of entities. Given the embeddings, many tools like FAISS \cite{Johnson2017}, and NMSLib \cite{Boytsov2013} \cite{Malkov2016} allow us to query the k most similar entities and their distances very efficiently. Moreover, it makes it perfect for Learning to Rank; a well-known Information Retrieval application \cite{McFee2010} \cite{Cakir2019}.

It is worth noting most Metric Learning research deals with a single entity type. One exception is Collaborative Filtering (CF) \cite{Schafer2007}, which learns the similarity between users and items. Even though people do not commonly recognize it as part of Metric Learning, they do arguably the same, the difference being that CF deals with two different entity types. There is even researching applying Triplet Network \cite{hoffer2018deep} to CF \cite{Tran2019} \cite{Liang2019}. Our inspiration to apply Triplet Network in this work came from there.

For the specific application of Metric Learning to rank labs-of-origin, we could not find any research. Previous work focused on creating a classifier, and no one else explored this idea before, to the best of our knowledge.
